Understanding Factors that Influence Upskilling

We investigate the motivation and means through which individuals expand their skill-set by analyzing a survey of applicants from the Facebook Jobs product. Individuals who report being influenced by their networks or local economy are over 29% more likely to have a postsecondary degree, but peer effects still exist among those who do not acknowledge such influences. Users with postsecondary degrees are more likely to upskill in general, by continuing coursework or applying to higher-skill jobs, though the latter is more common among users across all education backgrounds. These findings indicate that policies aimed at connecting individuals with different educational backgrounds can encourage upskilling. Policies that encourage users to enroll in coursework may not be as effective among individuals with a high school degree or less. Instead, connecting such individuals to opportunities that value skills acquired outside of a formal education, and allow for on-the-job training, may be more effective.

==> behavior_all.tex <==
\begin{table}[!htbp] \centering 
  \caption{Respondent Behavior} 
  \label{} 
 \scalebox{.8}{
 \begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
\\[-1.8ex] & \multicolumn{2}{c}{Applying for jobs post-survey} & \multicolumn{1}{c}{Continued-Edu (12 months)} \\ 
\\[-1.8ex] & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)}\\ 
\hline \\[-1.8ex] 
 Home-zipcode & 0.009 & 0.009 & 0.013 \\ 
Median Income ($\log$)    & (0.007) & (0.007) & (0.014) \\ 
  & & & \\ 
HS/GED & 0.010 & 0.009 & 0.025 \\ 
  & (0.008) & (0.008) & (0.019) \\ 
  & & & \\ 
2y College & 0.012 & 0.010 & 0.126^{***} \\ 
  & (0.008) & (0.009) & (0.021) \\ 
  & & & \\ 
BA/BSc & 0.014 & 0.012 & 0.114^{***} \\ 
  & (0.010) & (0.010) & (0.024) \\ 
  & & & \\ 
Graduate Degree & 0.014 & 0.013 & 0.248^{***} \\ 
  & (0.013) & (0.013) & (0.032) \\ 
  & & & \\ 
 Unemployed & 0.042^{***} & 0.039^{***} & 0.040^{***} \\ 
  & (0.007) & (0.007) & (0.014) \\ 
  & & & \\ 
Employed \&  & 0.020^{***} & 0.020^{***} & -0.0002 \\ 
looking  & (0.005) & (0.005) & (0.012) \\ 
  & & & \\ 
Share of friends &  & 0.00001 & 0.0001^{**} \\ 
with college degree  &  & (0.00002) & (0.00004) \\ 
  & & & \\ 
Thinks school-learned & 0.003 & 0.004 & 0.104^{***} \\ 
skills matter  & (0.006) & (0.006) & (0.014) \\ 
  & & & \\ 
 Network Influence & 0.016^{**} & 0.015^{**} & 0.049^{***} \\ 
  & (0.007) & (0.007) & (0.013) \\ 
  & & & \\ 
 Local Influence & -0.011^{**} & -0.010^{**} & 0.057^{***} \\ 
  & (0.005) & (0.005) & (0.011) \\ 
  & & & \\ 
\hline \\[-1.8ex] 
Dep. Mean & 0.17 & 0.17 & 0.24 \\ 
Observations & \multicolumn{1}{c}{9,568} & \multicolumn{1}{c}{9,568} & \multicolumn{1}{c}{9,568} \\ 
Log Likelihood & \multicolumn{1}{c}{1,985.531} & \multicolumn{1}{c}{1,994.476} & \multicolumn{1}{c}{-5,261.821} \\ 
Akaike Inf. Crit. & \multicolumn{1}{c}{-3,909.062} & \multicolumn{1}{c}{-3,914.952} & \multicolumn{1}{c}{10,589.640} \\ 
\hline 
\hline \\[-1.8ex] 
  \multicolumn{4}{l}{\textit{Note: All specifications also control for number of friends, gender and a quadratic polynomial  }}\\
    \multicolumn{4}{l}{\textit{of age. Robust standard errors in parentheses. $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} }\\

\end{tabular} }
\end{table} 

==> behavior_applicants.tex <==
\begin{table}[!htbp] \centering 
  \caption{Subsample: Still Applying for Jobs after Survey} 
  \label{} 
  \scalebox{.8}{
\begin{tabular}{@{\extracolsep{5pt}}lD{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
\\[-1.8ex] & \multicolumn{2}{c}{Upskilling} & \multicolumn{1}{c}{Continued-Edu (past 12 months)} \\ 
\\[-1.8ex] & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)}\\ 
\hline \\[-1.8ex] 
Home-zipcode & 0.073^{*} & 0.070^{*} & -0.017 \\ 
Median Income (log)  & (0.040) & (0.040) & (0.035) \\ 
  & & & \\ 
HS/GED & 0.107^{*} & 0.101^{*} & 0.036 \\ 
  & (0.056) & (0.056) & (0.045) \\ 
  & & & \\ 
2y College & 0.109^{*} & 0.102^{*} & 0.116^{**} \\ 
  & (0.059) & (0.059) & (0.049) \\ 
  & & & \\ 
BA/BSc & 0.186^{***} & 0.155^{**} & 0.083 \\ 
  & (0.069) & (0.069) & (0.059) \\ 
  & & & \\ 
Graduate Degree & 0.203^{**} & 0.178^{**} & 0.231^{***} \\ 
  & (0.086) & (0.087) & (0.073) \\ 
  & & & \\ 
Unemployed & 0.044 & 0.055 & -0.027 \\ 
  & (0.054) & (0.054) & (0.048) \\ 
  & & & \\ 
Employed \& & 0.063^{*} & 0.063^{*} & 0.027 \\ 
 Looking & (0.033) & (0.033) & (0.030) \\ 
  & & & \\ 
Thinks school-learned & -0.088^{**} & -0.078^{**} & 0.092^{***} \\ 
Matters  & (0.035) & (0.035) & (0.033) \\ 
  & & & \\ 
Is looking to &  & 0.045 & -0.029 \\ 
expand skillset  &  & (0.035) & (0.030) \\ 
  & & & \\ 
Has taken classes &  & -0.043 &  \\ 
lessons in the past 12 months  &  & (0.029) &  \\ 
  & & & \\ 
Share of current friends &  & 0.0003^{***} & 0.0002^{**} \\ 
with college degree  &  & (0.0001) & (0.0001) \\ 
  & & & \\ 
Network Influence & 0.019 & 0.014 & 0.064^{**} \\ 
  & (0.033) & (0.033) & (0.030) \\ 
  & & & \\ 
Local Influence & -0.018 & -0.014 & 0.049^{*} \\ 
  & (0.029) & (0.029) & (0.027) \\ 
  & & & \\ 
\# Educational & 0.0002 & 0.00003 & 0.001^{**} \\ 
Institutions in Home CZ  & (0.0005) & (0.0005) & (0.0005) \\ 
  & & & \\ 
Offer weekend & 0.029 & 0.023 & -0.017 \\ 
and night (share)  & (0.059) & (0.059) & (0.052) \\ 
  & & & \\ 
Offer remedial (share) & 0.130 & 0.140^{*} & 0.138^{**} \\ 
  & (0.079) & (0.079) & (0.068) \\ 
  & & & \\ 
\hline \\[-1.8ex] 
Dep. Mean & 0.42 & 0.42 & 0.25 \\ 
Observations & \multicolumn{1}{c}{1,687} & \multicolumn{1}{c}{1,687} & \multicolumn{1}{c}{1,687} \\ 
Log Likelihood & \multicolumn{1}{c}{-1,182.439} & \multicolumn{1}{c}{-1,174.850} & \multicolumn{1}{c}{-958.138} \\ 
Akaike Inf. Crit. & \multicolumn{1}{c}{2,426.877} & \multicolumn{1}{c}{2,421.700} & \multicolumn{1}{c}{1,984.276} \\ 
\hline 
\hline \\[-1.8ex] 
  \multicolumn{4}{l}{\textit{Note: All specifications also control for number of friends, gender and a quadratic polynomial  }}\\
    \multicolumn{4}{l}{\textit{of age. Robust standard errors in parentheses. $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} }\\
\end{tabular} }
\end{table} 
